The MICADO Atmospheric Dispersion Corrector: Optomechanical design, expected performance and calibration techniques

The differential refraction of light passing through the atmosphere can have a severe impact on image quality if no atmospheric dispersion corrector (ADC) is used. For the Extremely Large Telescope (ELT) this holds true well into the infrared. MICADO, the near-infrared imaging camera for the ELT, will employ a cryogenic ADC consisting of two counter-rotating Amici prisms with diameters of 125 mm. The mechanism will reduce the atmospheric dispersion to below 2.5 milli arcseconds (mas), with a set goal of 1 mas. In this report, we provide an overview of the current status of the ADC in development for MICADO. We summarise the optomechanical design and discuss how the cryogenic environment impacts the performance. We will also discuss our plan to use a diffraction mask in the cold pupil to calibrate and validate the performance once the instrument is fully integrated.

==> 04_expected_performance.tex <==
\section{EXPECTED PERFORMANCE}
% Should this include ScopeSIM simulations? Overview/budget of all residual dispersion effects. Some ZEMAX plots?
% Discussion of some of the prototype tests (performance and lifetime)
% Show measured wobble and discuss impact on performance
% Show images of wear and tear?
% Show temperature curves? Zettlex? "Step" response? Motor modelling?

